Provable Model Provenance Set for Large Language Models

The growing prevalence of unauthorized model usage and misattribution has increased the need for reliable model provenance analysis. However, existing methods largely rely on heuristic fingerprint-matching rules that lack provable error control and often overlook the existence of multiple sources, leaving the reliability of their provenance claims unverified. In this work, we first formalize the model provenance problem with provable guarantees, requiring rigorous coverage of all true provenances at a prescribed confidence level. Then, we propose the Model Provenance Set (MPS), which employs a sequential test-and-exclusion procedure to adaptively construct a small set satisfying the guarantee. The key idea of MPS is to test the significance of provenance existence within a candidate pool, thereby establishing a provable asymptotic guarantee at a user-specific confidence level. Extensive experiments demonstrate that MPS effectively achieves target provenance coverage while strictly limiting the inclusion of unrelated models, and further reveal its potential for practical provenance analysis in attribution and auditing tasks.

==> Sections/methodology.tex <==


\subsection{Algorithms}

\cref{alg:example} shows an example.

\begin{algorithm}[tb]
  \caption{Bubble Sort}
  \label{alg:example}
  \begin{algorithmic}
    \STATE {\bfseries Input:} data $x_i$, size $m$
    \REPEAT
    \STATE Initialize $noChange = true$.
    \FOR{$i=1$ {\bfseries to} $m-1$}
    \IF{$x_i > x_{i+1}$}
    \STATE Swap $x_i$ and $x_{i+1}$
    \STATE $noChange = false$
    \ENDIF
    \ENDFOR
    \UNTIL{$noChange$ is $true$}
  \end{algorithmic}
\end{algorithm}



\subsection{Theorems and Such}
The preferred way is to number definitions, propositions, lemmas, etc.
consecutively, within sections, as shown below.
\begin{definition}
  \label{def:inj}
  A function $f:X \to Y$ is injective if for any $x,y\in X$ different, $f(x)\ne
    f(y)$.
\end{definition}
Using \cref{def:inj} we immediate get the following result:
\begin{proposition}
  If $f$ is injective mapping a set $X$ to another set $Y$,
  the cardinality of $Y$ is at least as large as that of $X$
\end{proposition}
\begin{proof}
  Left as an exercise to the reader.
\end{proof}
\cref{lem:usefullemma} stated next will prove to be useful.
\begin{lemma}
  \label{lem:usefullemma}
  For any $f:X \to Y$ and $g:Y\to Z$ injective functions, $f \circ g$ is
  injective.
\end{lemma}
\begin{theorem}
  \label{thm:bigtheorem}
  If $f:X\to Y$ is bijective, the cardinality of $X$ and $Y$ are the same.
\end{theorem}
An easy corollary of \cref{thm:bigtheorem} is the following:
\begin{corollary}
  If $f:X\to Y$ is bijective,
  the cardinality of $X$ is at least as large as that of $Y$.
\end{corollary}
\begin{assumption}
  The set $X$ is finite.
  \label{ass:xfinite}
\end{assumption}
\begin{remark}
  According to some, it is only the finite case (cf. \cref{ass:xfinite}) that
  is interesting.
\end{remark}
%restatable

